Segment-and-Classify: ROI-Guided Generalizable Contrast Phase Classification in CT Using XGBoost

Purpose: To automate contrast phase classification in CT using organ-specific features extracted from a widely used segmentation tool with a lightweight decision tree classifier. Materials and Methods: This retrospective study utilized three public CT datasets from separate institutions. The phase prediction model was trained on the WAW-TACE (median age: 66 [60,73]; 185 males) dataset, and externally validated on the VinDr-Multiphase (146 males; 63 females; 56 unk) and C4KC-KiTS (median age: 61 [50.68; 123 males) datasets. Contrast phase classification was performed using organ-specific features extracted by TotalSegmentator, followed by prediction using a gradient-boosted decision tree classifier. Results: On the VinDr-Multiphase dataset, the phase prediction model achieved the highest or comparable AUCs across all phases (>0.937), with superior F1-scores in the non-contrast (0.994), arterial (0.937), and delayed (0.718) phases. Statistical testing indicated significant performance differences only in the arterial and delayed phases (p<0.05). On the C4KC-KiTS dataset, the phase prediction model achieved the highest AUCs across all phases (>0.991), with superior F1-scores in arterial/venous (0.968) and delayed (0.935) phases. Statistical testing confirmed significant improvements over all baseline models in these two phases (p<0.05). Performance in the non-contrast class, however, was comparable across all models, with no statistically significant differences observed (p>0.05). Conclusion: The lightweight model demonstrated strong performance relative to all baseline models, and exhibited robust generalizability across datasets from different institutions.

==> backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering
\caption{Distribution of CT scans across different anatomical coverage (CH: chest, ABD: abdomen, PEL: pelvis) and contrast phases (non-contrast, arterial, venous, delayed) for the WAW-TACE, VinDr-Multiphase, and C4KC-KiTS datasets. ``None'' denotes partial scans limited to specific organs, e.g., liver-only or kidney-only coverage. (*Note: `Delayed' phase is referred to as `Other' in VinDr-MultiPhase and `Late' in C4KC-KiTS)}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
                  & CH & ABD & PEL & CH-ABD & ABD-PEL & CH-ABD-PEL & None & Total ~~ \\
\midrule
~~ WAW-TACE \\
~~~~ Non-contrast &  0 & 146 &   0 &      3 &      41 &          8 &    2 &   200 ~~ \\
~~~~ Arterial     &  1 & 182 &   1 &      7 &      30 &          7 &    2 &   230 ~~ \\
~~~~ Venous       &  1 &  58 &   2 &      1 &     141 &         23 &    5 &   231 ~~ \\
~~~~ Delayed      &  1 & 164 &   0 &      0 &      27 &          0 &    1 &   193 ~~ \\
~~~~ Total        &  3 & 550 &   3 &     11 &     239 &         38 &   10 &   854 ~~ \\
\midrule
~~ Vin-Dr Multiphase \\
~~~~ Non-contrast &  0 &   0 &   0 &      0 &     154 &         29 &    0 &   183 ~~ \\
~~~~ Arterial     &  0 & 315 &   0 &      2 &     172 &          0 &    2 &   491 ~~ \\
~~~~ Venous       &  0 &  20 &   0 &      0 &     351 &         40 &    1 &   412 ~~ \\
~~~~ Delayed*     &  0 &  88 &   1 &      0 &       6 &          1 &    4 &   100 ~~ \\
~~~~ Total        &  0 & 423 &   1 &      2 &     683 &         70 &    7 &  1186 ~~ \\
\midrule
~~ C4KC-KiTS \\
~~~~ Non-contrast &  0 &  55 &   1 &      0 &      51 &          0 &    0 &   107 ~~ \\
~~~~ Arterial     &  0 &  88 &   1 &      1 &     100 &         18 &    2 &   210 ~~ \\
~~~~ Delayed*     &  0 &  31 &   7 &      0 &      53 &          0 &    0 &    91 ~~ \\
~~~~ Total        &  0 & 174 &   9 &      1 &     204 &         18 &    2 &   408 ~~ \\
\bottomrule
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\caption{Multiple Comparison of Means - Tukey HSD, FWER=0.05 - models tested on VinDr-Multiphase dataset. The table presents pairwise comparisons between group1 and group2: meandiff represents the difference in means (group2 - group1), p-adj is the adjusted p-value, lower and upper indicate the confidence interval bounds, and reject denotes whether the null hypothesis is rejected (True/False).}
\centering
% \resizebox{0.8\width}{!}{%
\begin{tabular}{@{}rr|ccccc@{}}
\toprule
~~               group1 &               group2 & meandiff &  p-adj &   lower &   upper & reject ~~ \\ \midrule
~~              mc3\_18 &         r2plus3d\_18 & -0.0809  &    0.0 & -0.1163 & -0.0456 &   True ~~ \\
~~              mc3\_18 &              r3d\_18 & -0.0438  & 0.0078 & -0.0792 & -0.0085 &   True ~~ \\
~~              mc3\_18 &              xgboost &  0.0152  & 0.6868 & -0.0201 &  0.0505 &  False ~~ \\
~~         r2plus3d\_18 &              r3d\_18 &  0.0371  & 0.0351 &  0.0018 &  0.0724 &   True ~~ \\
~~         r2plus3d\_18 &              xgboost &  0.0961  &    0.0 &  0.0608 &  0.1314 &   True ~~ \\
~~              r3d\_18 &              xgboost &   0.059  & 0.0001 &  0.0237 &  0.0943 &   True ~~ \\
\bottomrule
\end{tabular}
% }
\label{tab:stats_vindr}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering
\caption{Phase classification performance of models on the C4KC-KiTS dataset: XGBoost, ResNet3D 18-layer (r3d\_18), Mixed Convolution Network 18-layer (mc3\_18), and R(2+1)D 18-layer (r2plus1d\_18). Results are based on model ensembles, and evaluated using AUC, Sensitivity, Specificity, PPV, F1 Score, and Accuracy.}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
~~                  & AUC   & Sensitivity   & Specificity   & PPV       & F1-score  & Accuracy  ~~\\
\midrule
~~XGBoost \\
~~~~Non-contrast    & 0.994 & 0.981         & 0.996         & 0.990     & 0.985     & 0.981     ~~\\
~~~~Arterial/Venous & 0.994 & 0.961         & 0.974         & 0.975     & 0.968     & 0.961     ~~\\
~~~~Delayed         & 0.991 & 0.956         & 0.974         & 0.915     & 0.935     & 0.956     ~~\\
\midrule
~~r3d\_18 \\
~~~~Non-contrast    & 0.992 & 0.981         & 0.973         & 0.929     & 0.954     & 0.981     ~~\\
~~~~Arterial/Venous & 0.961 & 0.876         & 0.878         & 0.884     & 0.880     & 0.876     ~~\\
~~~~Delayed         & 0.926 & 0.670         & 0.917         & 0.701     & 0.685     & 0.670     ~~\\
\midrule
~~mc3\_18 \\  
~~~~Non-contrast    & 0.989 & 0.971         & 0.940         & 0.852     & 0.908     & 0.971     ~~\\
~~~~Arterial/Venous & 0.925 & 0.838         & 0.772         & 0.796     & 0.816     & 0.838     ~~\\
~~~~Delayed         & 0.862 & 0.406         & 0.911         & 0.569     & 0.474     & 0.406     ~~\\
\midrule
~~r2plus1d\_18 \\
~~~~Non-contrast    & 0.992 & 0.981         & 0.986         & 0.963     & 0.972     & 0.981     ~~\\
~~~~Arterial/Venous & 0.917 & 0.800         & 0.777         & 0.792     & 0.796     & 0.800     ~~\\
~~~~Delayed         & 0.877 & 0.494         & 0.867         & 0.517     & 0.505     & 0.494     ~~\\
\bottomrule
\end{tabular}
% }
\label{tab:results_c4kckits}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\caption{Multiple Comparison of Means - Tukey HSD, FWER=0.05 - models tested on C4KC-KiTS dataset. The table presents pairwise comparisons between group1 and group2: meandiff represents the difference in means (group2 - group1), p-adj is the adjusted p-value, lower and upper indicate the confidence interval bounds, and reject denotes whether the null hypothesis is rejected (True/False).}
\centering
% \resizebox{0.8\width}{!}{%
\begin{tabular}{@{}rr|ccccc@{}}
\toprule
~~               group1 &               group2 & meandiff &  p-adj &   lower &   upper & reject ~~ \\ \midrule
~~              mc3\_18 &         r2plus1d\_18 &  0.0025  & 0.9997 & -0.0613 &  0.0662 &  False ~~ \\
~~              mc3\_18 &              r3d\_18 &  0.0809  & 0.0062 &  0.0171 &  0.1446 &   True ~~ \\
~~              mc3\_18 &              xgboost &  0.1887  &    0.0 &   0.125 &  0.2525 &   True ~~ \\
~~         r2plus1d\_18 &              r3d\_18 &  0.0784  & 0.0086 &  0.0147 &  0.1422 &   True ~~ \\
~~         r2plus1d\_18 &              xgboost &  0.1863  &    0.0 &  0.1225 &    0.25 &   True ~~ \\
~~              r3d\_18 &              xgboost &  0.1078  & 0.0001 &  0.0441 &  0.1716 &   True ~~ \\
\bottomrule
\end{tabular}
% }
\label{tab:stats_c4kckits}
\end{table}
